LLM-based Agent Simulation for Maternal Health Interventions: Uncertainty Estimation and Decision-focused Evaluation

Agent-based simulation is crucial for modeling complex human behavior, yet traditional approaches require extensive domain knowledge and large datasets. In data-scarce healthcare settings where historic and counterfactual data are limited, large language models (LLMs) offer a promising alternative by leveraging broad world knowledge. This study examines an LLM-driven simulation of a maternal mobile health program, predicting beneficiaries' listening behavior when they receive health information via automated messages (control) or live representatives (intervention). Since uncertainty quantification is critical for decision-making in health interventions, we propose an LLM epistemic uncertainty estimation method based on binary entropy across multiple samples. We enhance model robustness through ensemble approaches, improving F1 score and model calibration compared to individual models. Beyond direct evaluation, we take a decision-focused approach, demonstrating how LLM predictions inform intervention feasibility and trial implementation in data-limited settings. The proposed method extends to public health, disaster response, and other domains requiring rapid intervention assessment under severe data constraints. All code and prompts used for this work can be found at https://github.com/sarahmart/LLM-ABS-ARMMAN-prediction.

==> notes.tex <==
TODO: 

1. Calculate total accuracy over time for each model → put this in a table
2. Also do for only the first x weeks 
3. How to frame the fact that direct averaging and uncertainty-weighted perform basically exactly the same? see below
4. How can we check robustness? → confusion matrix? [how can we show that the extreme case is less likely, less likely to make serious mistakes, lowest accuracy is higher than the lowest accuracy of other models]
5. Fix graphs 
6. What other fine-grained analysis could be useful / interesting to see?
--> SHOULD LOOK AT SCENARIOS WHERE DIFFERENT ARMS DO NOT AGREE. DOES THE AGGREGATION FIX THESE PROBLEMS?

many similar predictions for the same arm ==> model lacks diversity in outputs 
uncertainty estimated by LLM is not accuracted, uncertainty not calibrated (reference this) --> important area for future research
many cases where predictive uncertainty = aleotoric, so epistemic uncertainty is low 

need to add some analysis of this 
Are there specific mothers who this affects more ? / where this is more common ?

initial predictions : on the CONTROL group !! not random 
intervention predictions on the random group 

%%%%%%%%%%%%%%%%%%%%%%%%%%

OPTIONS FOR INTERVENTION APPRAISAL

Random Selection Baseline: Compare the targeted intervention strategy against a random selection baseline. 

If targeting high-uncertainty or low-engagement mothers yields better engagement post-intervention, it justifies intentional selection over random allocation.

Compare simulated intervention selection to the real-world selection (any same mothers selected)

[run 2 more LLM simulations, one where I randomly intervene on k mothers per timestep and predict their engagement on and after intervention. and the second where I do some selection of the k mothers per timestep (using say the hybrid approach) to select k mothers per timestep and continue predicting on them? ]

Then compare the overall resulting engagement of these 2 settings to the true increase in engagement and to the baseline engagement with no intervention

[could also do feature weighting for selection ]

%%%%%%%%%%%%%%%%%%%%%%%%%%


SIMULATION NEVER INDICATES ACTUAL CHANGE IN SITUATION RELATED TO MESSAGES. ONLY LISTENING TIMES BUT NOT ACTUAL IMPROVEMENT

like a human, LLM might need some indication of a reward with long-term listening. Currently some reasoning indicates lack of change as a reason for not listening. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
